Estimating Self-Sustainability in Peer-to-Peer Swarming Systems

Peer-to-peer swarming is one of the \emph{de facto} solutions for distributed content dissemination in today's Internet. By leveraging resources provided by clients, swarming systems reduce the load on and costs to publishers. However, there is a limit to how much cost savings can be gained from swarming; for example, for unpopular content peers will always depend on the publisher in order to complete their downloads. In this paper, we investigate this dependence. For this purpose, we propose a new metric, namely \emph{swarm self-sustainability}. A swarm is referred to as self-sustaining if all its blocks are collectively held by peers; the self-sustainability of a swarm is the fraction of time in which the swarm is self-sustaining. We pose the following question: how does the self-sustainability of a swarm vary as a function of content popularity, the service capacity of the users, and the size of the file? We present a model to answer the posed question. We then propose efficient solution methods to compute self-sustainability. The accuracy of our estimates is validated against simulation. Finally, we also provide closed-form expressions for the fraction of time that a given number of blocks is collectively held by peers.

==> abstract.tex <==
\begin{abstract}
Peer-to-peer swarming is one of the \emph{de facto} solutions for distributed content dissemination in today's Internet.  By leveraging resources provided by clients, swarming systems reduce the load on and costs to publishers.  However, there is a limit to how much cost savings can be gained from swarming; for example, for  unpopular content peers will always depend on the publisher in order to complete their downloads.  In this paper, we investigate this  dependence.  For this purpose, we propose a new metric, namely \emph{swarm self-sustainability}.   A swarm is referred to as self-sustaining if all its blocks are collectively held by peers; the self-sustainability  of a swarm is the fraction of time in which the swarm is self-sustaining.    We pose the following question: how does the self-sustainability of a swarm vary as a function of  content popularity, the service capacity of the users, and the size of the file? We present a model to answer the posed question.  We then propose efficient solution methods to compute self-sustainability.  The accuracy of our estimates is validated against simulation. Finally, we also provide   closed-form expressions for  the fraction of time that a given number of blocks is  collectively held by peers. \end{abstract}





\begin{comment}
\begin{abstract}
The key problem addressed in this paper is how to estimate the  bandwidth incurred by content providers leveraging peer-to-peer swarming techniques.  \eat{
We consider publishers that use peer-to-peer systems to deliver content but that can afford a stable server (seed). }  \eat{In the realm of  hybrid peer-to-peer systems for enterprise content delivery,} We pose the following question:  what is the bandwidth consumed by a publisher  as a function of the  content popularity and the capacity of the users? The primary contribution of this paper is a model to answer the posed question.   We propose efficient solution methods to obtain the metrics of interest, namely the bandwidth consumed by the publisher and the fraction of chunks unavailable among the peers,  in scenarios of practical interest.  Finally, we  evaluate the accuracy of our model against experiments.




Peer-to-peer systems have the potential to revolutionize enterprise content distribution, but the widespread use of these systems is likely to happen only after some important  challenges are addressed.   For instance, peer-to-peer systems are usually assumed  not to be suited for the dissemination of unpopular content.   Nevertheless, making both popular and unpopular titles available is essential for a content delivery enterprise to thrive.  


Peer-to-peer systems have the potential to revolutionize enterprise content distribution, but the widespread use of these systems is likely to happen only after some important  challenges are addressed.   For instance, peer-to-peer systems are usually assumed  not to be suited for the dissemination of unpopular content.   Nevertheless, making both popular and unpopular titles available is essential for a content delivery enterprise to thrive.  The key question we answer in this paper is: how to estimate the minimum publishing costs, in terms of bandwidth, incurred by content providers?   In the realm of enterprise businesses that can afford a stable seed to deliver content to its users,  we pose the following two questions: 1) given the current number of users in the system, what is the estimated bandwidth consumed by the publisher? 2) in steady state, what is the minimum bandwidth consumed by the publisher as a function of the  content popularity and the capacity of the users? \eat{.   In the context of home publishers, that cannot afford a stable seed, we are interested in the regime in which peers can download  contents even in the absence of a seed, and consider the minimum content popularity above which a swarm may be considered self sustaining. }   \eat{  Once the question is answered, the publisher may decide, for instance, for which contents a third party enterprise should be used.  }  \eat{To answer this question, } The primary contribution of this paper is a model to answer the questions posed above.   \eat{estimate the publishing distribution costs for enterprise content delivery.  }    We propose efficient solution methods to solve our model in scenarios of practical interest, even when faced with a large state space.  Finally, we  evaluate the accuracy of our model against experiments.

\end{abstract}


\end{comment}


==> algorithmic.sty.1 <==
% ALGORITHMIC STYLE -- Released 8 APRIL 1996
%    for LaTeX version 2e
% Copyright -- 1994 Peter Williams
% E-mail PeterWilliams@dsto.defence.gov.au
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{algorithmic}
\typeout{Document Style `algorithmic' - environment}
%
\RequirePackage{ifthen}
\RequirePackage{calc}
\newboolean{ALC@noend}
\setboolean{ALC@noend}{false}
\newcounter{ALC@line}
\newcounter{ALC@rem}
\newlength{\ALC@tlm}
%
\DeclareOption{noend}{\setboolean{ALC@noend}{true}}
%
\ProcessOptions
%
% ALGORITHMIC
\newcommand{\algorithmicinput}{\textbf{Input:}}
\newcommand{\algorithmicoutput}{\textbf{Output:}}
\newcommand{\algorithmiccomment}[1]{\{#1\}}
\newcommand{\algorithmicend}{\textbf{end}}
\newcommand{\algorithmicif}{\textbf{if}}
\newcommand{\algorithmicthen}{\textbf{then}}
\newcommand{\algorithmicelse}{\textbf{else}}
\newcommand{\algorithmicelsif}{\algorithmicelse\ \algorithmicif}
\newcommand{\algorithmicendif}{\algorithmicend\ \algorithmicif}
\newcommand{\algorithmicfor}{\textbf{for}}
\newcommand{\algorithmicforall}{\textbf{for all}}
\newcommand{\algorithmicdo}{\textbf{do}}
\newcommand{\algorithmicendfor}{\algorithmicend\ \algorithmicfor}
\newcommand{\algorithmicwhile}{\textbf{while}}
\newcommand{\algorithmicendwhile}{\algorithmicend\ \algorithmicwhile}
\newcommand{\algorithmicloop}{\textbf{loop}}
\newcommand{\algorithmicendloop}{\algorithmicend\ \algorithmicloop}
\newcommand{\algorithmicrepeat}{\textbf{repeat}}
\newcommand{\algorithmicuntil}{\textbf{until}}
\def\ALC@item[#1]{%
\if@noparitem \@donoparitem
  \else \if@inlabel \indent \par \fi
         \ifhmode \unskip\unskip \par \fi
         \if@newlist \if@nobreak \@nbitem \else
                        \addpenalty\@beginparpenalty
                        \addvspace\@topsep \addvspace{-\parskip}\fi
           \else \addpenalty\@itempenalty \addvspace\itemsep
          \fi
    \global\@inlabeltrue
\fi
\everypar{\global\@minipagefalse\global\@newlistfalse
          \if@inlabel\global\@inlabelfalse \hskip -\parindent \box\@labels
             \penalty\z@ \fi
          \everypar{}}\global\@nobreakfalse
\if@noitemarg \@noitemargfalse \if@nmbrlist \refstepcounter{\@listctr}\fi \fi
\sbox\@tempboxa{\makelabel{#1}}%
\global\setbox\@labels
 \hbox{\unhbox\@labels \hskip \itemindent
       \hskip -\labelwidth \hskip -\ALC@tlm
       \ifdim \wd\@tempboxa >\labelwidth
                \box\@tempboxa
          \else \hbox to\labelwidth {\unhbox\@tempboxa}\fi
       \hskip \ALC@tlm}\ignorespaces}
%
\newenvironment{algorithmic}[1][0]{
\let\@item\ALC@item
  \newcommand{\ALC@lno}{%
\ifthenelse{\equal{\arabic{ALC@rem}}{0}}
{{\footnotesize \arabic{ALC@line}:}}{}%
}
\let\@listii\@listi
\let\@listiii\@listi
\let\@listiv\@listi
\let\@listv\@listi
\let\@listvi\@listi
\let\@listvii\@listi
  \newenvironment{ALC@g}{
    \begin{list}{\ALC@lno}{ \itemsep\z@ \itemindent\z@
    \listparindent\z@ \rightmargin\z@ 
    \topsep\z@ \partopsep\z@ \parskip\z@\parsep\z@
    \leftmargin 1em
    \addtolength{\ALC@tlm}{\leftmargin}
    }
  }
  {\end{list}}
  \newcommand{\ALC@it}{\addtocounter{ALC@line}{1}\addtocounter{ALC@rem}{1}\ifthenelse{\equal{\arabic{ALC@rem}}{#1}}{\setcounter{ALC@rem}{0}}{}\item}
  \newcommand{\ALC@com}[1]{\ifthenelse{\equal{##1}{default}}%
{}{\ \algorithmiccomment{##1}}}
  \newcommand{\INPUT}{\item[\algorithmicinput]}
  \newcommand{\OUTPUT}{\item[\algorithmicoutput]}
  \newcommand{\STATE}{\ALC@it}
  \newcommand{\COMMENT}[1]{\algorithmiccomment{##1}}
  \newenvironment{ALC@if}{\begin{ALC@g}}{\end{ALC@g}}
  \newenvironment{ALC@for}{\begin{ALC@g}}{\end{ALC@g}}
  \newenvironment{ALC@whl}{\begin{ALC@g}}{\end{ALC@g}}
  \newenvironment{ALC@loop}{\begin{ALC@g}}{\end{ALC@g}}
  \newenvironment{ALC@rpt}{\begin{ALC@g}}{\end{ALC@g}}
  \renewcommand{\\}{\@centercr}
  \newcommand{\IF}[2][default]{\ALC@it\algorithmicif\ ##2\ \algorithmicthen%
\ALC@com{##1}\begin{ALC@if}}
  \newcommand{\ELSE}[1][default]{\end{ALC@if}\ALC@it\algorithmicelse%
\ALC@com{##1}\begin{ALC@if}}
  \newcommand{\ELSIF}[2][default]%
{\end{ALC@if}\ALC@it\algorithmicelsif\ ##2\ \algorithmicthen%
\ALC@com{##1}\begin{ALC@if}}
  \newcommand{\FOR}[2][default]{\ALC@it\algorithmicfor\ ##2\ \algorithmicdo%
\ALC@com{##1}\begin{ALC@for}}
  \newcommand{\FORALL}[2][default]{\ALC@it\algorithmicforall\ ##2\ %
\algorithmicdo%
\ALC@com{##1}\begin{ALC@for}}
  \newcommand{\WHILE}[2][default]{\ALC@it\algorithmicwhile\ ##2\ %
\algorithmicdo%
\ALC@com{##1}\begin{ALC@whl}}
  \newcommand{\LOOP}[1][default]{\ALC@it\algorithmicloop%
\ALC@com{##1}\begin{ALC@loop}}
  \newcommand{\REPEAT}[1][default]{\ALC@it\algorithmicrepeat%
\ALC@com{##1}\begin{ALC@rpt}}
  \newcommand{\UNTIL}[1]{\end{ALC@rpt}\ALC@it\algorithmicuntil\ ##1}
  \ifthenelse{\boolean{ALC@noend}}{
    \newcommand{\ENDIF}{\end{ALC@if}}
    \newcommand{\ENDFOR}{\end{ALC@for}}
    \newcommand{\ENDWHILE}{\end{ALC@whl}}
    \newcommand{\ENDLOOP}{\end{ALC@loop}}
  }{
    \newcommand{\ENDIF}{\end{ALC@if}\ALC@it\algorithmicendif}
    \newcommand{\ENDFOR}{\end{ALC@for}\ALC@it\algorithmicendfor}
    \newcommand{\ENDWHILE}{\end{ALC@whl}\ALC@it\algorithmicendwhile}
    \newcommand{\ENDLOOP}{\end{ALC@loop}\ALC@it\algorithmicendloop}
  } 
  \renewcommand{\@toodeep}{}
  \begin{list}{\ALC@lno}{\setcounter{ALC@line}{0}\setcounter{ALC@rem}{0}%
    \itemsep\z@ \itemindent\z@ \listparindent\z@%
    \partopsep\z@ \parskip\z@ \parsep\z@%
    \labelsep 0.5em \topsep 0.2em%
\ifthenelse{\equal{#1}{0}}
  {\labelwidth 0.5em }
  {\labelwidth  1.2em }
\leftmargin\labelwidth \addtolength{\leftmargin}{\labelsep}
    \ALC@tlm\labelsep
  }
}
{\end{list}}


==> intro.tex <==
\section{Introduction}

Peer-to-peer swarming, such as used by \eat{the immensely popular} BitTorrent~\cite{bt}, is a  scalable and efficient way to publish   content in today's Internet.  Peer-to-peer swarming has been widely studied during the last decade, and its use by enterprises is steadily growing~\cite{warner, twitter, amazon, ubuntu}.  \eat{In essence, the popularity of peer-to-peer swarming occurs because it allows  publishers to  provide a large number of files to clients, at a low cost. }  By leveraging resources provided by clients, peer-to-peer swarming  decreases costs to publishers, and provides scalability and system robustness.  As  demand for content increases, system capacity scales accordingly, as all clients collaborate with each other while downloading the desired content.  As the demand for multimedia files and the size of these files increase, peer-to-peer swarming systems have become an important content dissemination solution for many content providers~\cite{amazon,ubuntu}. 
 
 \eat{
Although peer-to-peer swarming systems are a powerful tool for content delivery, the  vast majority  of publishers  adopts client-server strategies.  Indeed, there are still a number of challenges to be addressed before peer-to-peer swarming systems will be widely adopted.   \eat{For instance, publishers have worried that the use of peer-to-peer systems can hinder simple billing and copyright enforcement mechanisms.    Native support for electronic sales and advertisement in peer-to-peer systems~\cite{vuze} is an initial step to meet the monetization needs, whereas automated auditors~\cite{sherman, p2ppolice} and digital right mechanisms (DRM)~\cite{drm} have been suggested to meet the copyright requirements.   

}  }


However, there is a limit on how much savings can be gained from swarming techniques.  For example, in the case of unpopular content, peers must  rely on the publisher in order to complete their downloads. In this paper, we investigate such a dependence of peers on a publisher. \eat{, willing to  provide an extensive catalog of titles, that include unpopular ones~\cite{anderson}.  }

A swarm is a set of peers interested in the same content (file or bundle of files~\cite{mainarticle}) that exchange \eat{(download and upload) } blocks of the files among themselves.    We consider a scenario where each swarm includes one stable publisher that is always online and ready to serve content.  The corresponding system is henceforth referred to as a hybrid peer-to-peer system, since peers can always rely on the publisher if they cannot find blocks of the files  among themselves. \eat{ (content is always available). } If all blocks are \sustained, \eat{excluding the publisher, } the swarm is referred to as \emph{self-sustaining}.   Quantifying \eat{the } swarm self-sustainability, defined as the fraction of time during  which the swarm is self-sustaining, is useful for provisioning purposes.  The larger the swarm's self-sustainability, \eat{which depends on the popularities of the files and the capacity of the peers,} the lower the dependency of peers on the publisher, and the lower the  bandwidth needed by the publisher to serve~the~peers.  \eat{Given a bandwidth capacity constraint at  the publisher,  swarm self-sustainability can also be used for dimensioning purposes, to determine the number of swarms that the publisher is able to serve. \eat{handle.  }}

The primary contribution of this paper is  a model to study   \eat{the dependency of peers on  publishers in peer-to-peer swarming systems.  The dependecy is measured as the } swarm  self-sustainability.    We use a two-layer model to quantify  swarm \eat{fraction of time in which a swarm is self-sustaining } self-sustainability as a function of the number of blocks in the file, the mean upload capacity of peers and the popularity of a file.   The upper layer of our model  captures the evolution of user dynamics over time, while  the lower layer  captures the availability of blocks among the peers given an upper layer state.  Our model is flexible enough to account for any number of blocks in the file, heterogeneous download times for different blocks, and peers residing in the system after completing their downloads.   We derive closed-form expressions for the distribution of the number of \bsustained{}   \eat{ to solve the proposed model.  }     \eat{Then, we provide probabilistic interpretation for the closed-form expressions,}  and apply them to show that \eat{for a given mean user capacity and file popularity,  the} self-sustainability increases as a function of the number of blocks in the file. \eat{ Nevertheless, the closed-form } The derived expressions involve sums and subtractions of large numbers, and are amenable to numerical errors.   Hence,  we present an efficient algorithm to compute the swarm self-sustainability that  avoids these problems.
We \eat{apply our solution algorithm to } then numerically investigate the minimum popularity needed to attain a given self-sustainability level. \eat{, and observe that the log of the minimum  popularity is linear in the log of the file size.   } Finally, we validate the estimates made by the model against detailed simulations. 
  


\begin{comment}
In summary, we make the following contributions,


\textbf{Self-sustainability model:}  We present a model of   self-sustainability for peer-to-peer swarming.     \eat{in swarming systems.} \eat{To our knowledge, our model is the first to quantify the self-sustainability of a swarm}  
 Using the model, we derive closed-form expressions to compute the fraction of time that a given fraction of blocks is collectively held by peers as a function  of the number of blocks in the file, mean service capacity of peers, and content popularity. 

\textbf{Efficient solution technique:} Starting from our model, we propose an efficient, to compute the self-sustainability of a swarm.  

\textbf{Numerical evaluation:}   Using our efficient solution technique, we numerically study the minimum content popularity  necessary to attain a given self-sustainability level.  


 \eat{The algorithm is convenient to avoid numerical problems since, in contrast to the closed-form expressions, it requires only sums and multiplications of probabilities.} \eat{We validate the estimates made by the model against simulations which show the accuracy of our model.  Our simulations also show that the metrics obtained with our model hold even when we relax some of the model assumptions.} \eat{, allowing for realistic arrival patterns and upload capacities.  }
\end{comment}

The remainder of this paper is organized as follows.  After providing a  background into swarming systems in~\textsection\ref{sec:primer},  \eat{ and exemplify using measurements some of the difficulties that may be faced by publishers relying on swarming systems to disseminate content. } \eat{in~\textsection\ref{sec:motivate} we further motivate the problem considered in this paper  and} we propose our model in \textsection\ref{sec:model}.  In \textsection\ref{sec:instant} \eat{and \textsection\ref{sec:bawsteady} } we present an efficient algorithm to solve the proposed model followed by analytical results in~\textsection{\ref{sec:analytical}}. \eat{, respectively. } In \textsection\ref{sec:exp} we evaluate our model against experiments. In \textsection\ref{assumptions} we discuss some limitations and caveats of our model,   \textsection\ref{sec:related} presents the related work and \textsection\ref{sec:conclusion} concludes the paper.   






